Vehicle lateral control using Machine Learning for automated vehicle guidance

Uncertainty in decision-making is crucial in the machine learning model used for a safety-critical system that operates in the real world. Therefore, it is important to handle uncertainty in a graceful manner for the safe operation of the CPS. In this work, we design a vehicle's lateral controller using a machine-learning model. To this end, we train a random forest model that is an ensemble model and a deep neural network model. Due to the ensemble in the random forest model, we can predict the confidence/uncertainty in the prediction. We train our controller on data generated from running the car on one track in the simulator and tested it on other tracks. Due to prediction in confidence, we could decide when the controller is less confident in prediction and takes control if needed. We have two results to share: first, even on a very small number of labeled data, a very good generalization capability of the random forest-based regressor in comparison with a deep neural network and accordingly random forest controller can drive on another similar track, where the deep neural network-based model fails to drive, and second confidence in predictions in random forest controller makes it possible to let us know when the controller is not confident in prediction and likely to fail. By creating a threshold, it was possible to take control when the controller is not safe and that is missing in a deep neural network-based controller.

==> acknowledgement.tex <==
\section{Acknowledgments}
This work at Vanderbilt University was supported in part by the PIRE program of NSF under award \#1743772 and by National Institute of Standards and Technology under award 70NANB18H269.

